Lossless White Balance For Improved Lossless CFA Image and Video Compression

Color filter array is spatial multiplexing of pixel-sized filters placed over pixel detectors in camera sensors. The state-of-the-art lossless coding techniques of raw sensor data captured by such sensors leverage spatial or cross-color correlation using lifting schemes. In this paper, we propose a lifting-based lossless white balance algorithm. When applied to the raw sensor data, the spatial bandwidth of the implied chrominance signals decreases. We propose to use this white balance as a pre-processing step to lossless CFA subsampled image/video compression, improving the overall coding efficiency of the raw sensor data.

==> 4-3_shift_lifting.tex <==
\subsection{Lifting Based Shift Transform}
\label{sec:shiftLifting}
The analysis in \sref{sec:cfaSampling} implies that the wavelet coefficients of $w_{\scriptscriptstyle LH}^{x}$, $w_{\scriptscriptstyle HL}^{x}$, and $w_{\scriptscriptstyle HH}^{x}$ are dominated by lowpass components, which yields poor coding efficiency. Recalling (\ref{eq:waveletCoeff_2}), the wavelet coefficients of $w_{\scriptscriptstyle LL^\ast}^{\gamma}$ and  $w_{\scriptscriptstyle L^\ast L}^{\gamma}$ are the approximation coefficients of the same chrominance frame $\gamma$. This suggests that $w_{\scriptscriptstyle LH}^{x}$ and $w_{\scriptscriptstyle HL}^{x}$ are highly correlated. % as shown in \fref{fig:comparisonDWT}(c). 
One key contribution to lossless CAMRA compression was to decorrelate by subtracting $w_{\scriptscriptstyle LL^\ast}^{\gamma}$ from $w_{\scriptscriptstyle L^\ast L}^{\gamma}$~\cite{lee2018camera}:
\begin{align}\label{eq:CAMRA1}
    \begin{split}
    r^{x}=&w^{x}_{\scriptscriptstyle LH}-w^{x}_{\scriptscriptstyle HL}=(w^{\ell}_{\scriptscriptstyle LH}-w^{\ell}_{\scriptscriptstyle HL})+(w^{\gamma}_{\scriptscriptstyle LL^*}-w^{\gamma}_{\scriptscriptstyle L^*L})\vspace{0.3cm}\\
    s^{x}=&\left\lfloor\frac{w^{x}_{\scriptscriptstyle LH}+w^{x}_{\scriptscriptstyle HL}}{2}\right\rfloor,
    \end{split}
\end{align}
where $\lfloor \cdot \rfloor$ denotes a {\it floor} operation.

However, recall that the scaling function ($L$) and wavelet function ($H$) of LeGall 5/3 transform are $[-\frac{1}{8},\frac{1}{4},\mathbf{\frac{3}{4}},\frac{1}{4},-\frac{1}{8}]$ and $[-\frac{1}{2},\mathbf{1},-\frac{1}{2},0,0]$, respectively. The amplitude modulation of chrominance component $\gamma(i,j)$
stemming from CFA sampling results in a conjugate LeGall 5/3 transforms $w^{\gamma}_{LL^*}$ and $w^{\gamma}_{L^*L}$, with the corresponding conjugate scaling function ($L^*$) of the form $[\frac{1}{2},\mathbf{1},\frac{1}{2},0,0]$. The centers of symmetries (highlighted in {\bf bold font}) of $L$ and $L^*$ scaling coefficients occur on even and odd samples, respectively---meaning they are shifted by one pixel location, relative to each other. Hence, the implied relative pixel misalignment between $LL^*$ and $L^*L$ is $[1,-1]$ in the CFA image domain. Or equivalently, the shift is $[\frac{1}{2},\frac{-1}{2}]$ in the wavelet domain (due to the downsampling by factor of 2 that occurs in wavelet transform)---that is, 
$w^{\gamma}_{LL^*}(i,j+\frac{1}{2})\approx w^{\gamma}_{L^*L}(i+\frac{1}{2},j)$.
In order for the wavelet transform to be reversible, this implied misalignment by $\|[\frac{1}{2},\frac{-1}{2}]\|=\sqrt{1/2}$ is a necessary inconvenience.

The residual term $w^{\gamma}_{LL^*}-w^{\gamma}_{L^*L}$ in $r(i,j)$ as described in \eqref{eq:CAMRA1} represents a difference of two misaligned chrominance wavelet components, which acts more like a bandpass filter applied to the chrominance image than a decorrelation. While this bandpass filter suppresses the lowpass component of $w^{\gamma}_{LL^*}$, the nontrivial residual signal as observed in \fref{fig:residual}(a) worsens coding efficiency. One way to handle this residual is to apply a further spatial transformation to sparsify the residuals~\cite{lee2018camera}. However, it comes at the cost of increasing the dynamic range of the transformed coefficients~\cite{Adams00}, limiting the effectiveness of the lossless CAMRA compression performance. 

Consequently, we develop a new CAMRA decorrelation strategy that takes misalignment into account. In order to sparsify $w_{\scriptscriptstyle LH}^{x}$ and $w_{\scriptscriptstyle HL}^{x}$ with minimal dynamic range increase, we propose to spatially register $w_{LL^*}^{\gamma}$ and $w_{L^*L}^{\gamma}$ using a lifting scheme based shift transform. We perform the following transformation~(See \fref{fig:losslessShifting}): 
\begin{align}\label{eq:lifting}
\begin{array}{l}
u^{x}(i,j) = w_{\scriptscriptstyle LH}^{x}(i,j) - \Bigl\lfloor S_1\Bigl( w_{\scriptscriptstyle HL}^{x}(ii,jj) \Bigr)\Bigr\rfloor \vspace{0.1cm}\\
v^{x}(i,j) = w_{\scriptscriptstyle HL}^{x}(i,j) + \Bigl\lfloor S_2\Bigl( u^{x}(ii,jj) \Bigr) \Bigr\rfloor,
\end{array}\end{align}
where  $(ii,jj) \in \Omega$ are pixel locations in the region $\Omega$ in the vicinity of $(i,j)$; $S_1(\cdot)$ is an operation that helps sparsifing wavelet coefficient, and $S_2(\cdot)$ is a transformation that further cancels out the highpass signals. The transformations $S_1$ and $S_2$ can be implemented as the predict and update operations in \fref{fig:liftingDWT}, respectively. In predict operation, we let the transformation $S_1(\cdot)$ be the interpolation function to estimate the ``subpixel values'' of $w_{\scriptscriptstyle HL}^{x}$ at locations $(i+\frac{1}{2},j-\frac{1}{2})$ so as to align $w_{L^*L}^{\gamma}$ to $w_{LL^*}^{\gamma}$. To further smooth luminance components $w_{\scriptscriptstyle LH}^{\ell}$ and $w_{\scriptscriptstyle HL}^{\ell}$, the update operation $S_2(\cdot)$ cancels out the highpass signals. Owing to the lifting structure, any arbitrary linear transformations $S_1$ and $S_2$ are perfectly reconstructable from $u^{x}$ and $v^{x}$, as follows:
\begin{align}\begin{array}{l}
w_{\scriptscriptstyle HL}^{x}(i,j) = v^{x}(i,j) - \Bigl\lfloor S_2\Bigl( u^{x}(ii,jj) \Bigr) \Bigr\rfloor \vspace{0.2cm}\\
w_{\scriptscriptstyle LH}^{x}(i,j) = u^{x}(i,j) +  \Bigl\lfloor S_1\Bigl( w_{\scriptscriptstyle HL}^{x}(ii,jj) \Bigr)\Bigr\rfloor .
\end{array}\end{align}
Modeled after LeGall 5/3 transform, the predict and update operations by $S_1$ and $S_2$ are linear filtering by %$[\frac{1}{2},\mathbf{\frac{1}{2}},0]^T\cdot[0\:\:\frac{1}{2}\:\:\frac{1}{2}]$ and $[0\:\:\frac{1}{4}\:\:\frac{1}{4}]^T\cdot[\frac{1}{4}\:\:\frac{1}{4}\:\:0]$, 
$[0;\frac{1}{2};\frac{1}{2}]\cdot[\frac{1}{2},\frac{1}{2},0]$ and $[\frac{1}{4};\frac{1}{4};0]\cdot[0,\frac{1}{4},\frac{1}{4}]$ in our implementation, 
respectively. In addition to shifting, the averaging nature of the $S_1$ and $S_2$ transformation help reduce noise in $u^{x}$ and $v^{x}$.

==> f_lossless_shift.tex <==
% Fig. 5
\begin{figure*}[!t]
    \begin{minipage}{0.49\linewidth}
    \centering
    \centerline{\includegraphics[scale=0.45]{lossless_shift}}
    \centerline{\footnotesize{(a)}}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
    \centerline{\includegraphics[scale=0.45]{inverse_lossless_shift}}
    \centerline{\footnotesize{(b)}}
    \end{minipage}
    \caption{Lifting-based CAMRA for CFA compression proposed in \sref{sec:shiftLifting}. (a) Forward transform. (b) Inverse transform. $P$ and $U$ denote a predict operation and a update operation, respectively.}   \label{fig:losslessShifting}
\end{figure*}

